SEMULATOR: Emulating the Dynamics of Crossbar Array-based Analog Neural System with Regression Neural Networks

As deep neural networks require tremendous amount of computation and memory, analog computing with emerging memory devices is a promising alternative to digital computing for edge devices. However, because of the increasing simulation time for analog computing system, it has not been explored. To overcome this issue, analytically approximated simulators are developed, but these models are inaccurate and narrow down the options for peripheral circuits for multiply-accumulate operation (MAC). In this sense, we propose a methodology, SEMULATOR (SiMULATOR by Emulating the analog computing block) which uses a deep neural network to emulate the behavior of crossbar-based analog computing system. With the proposed neural architecture, we experimentally and theoretically shows that it emulates a MAC unit for neural computation. In addition, the simulation time is incomparably reduced when it compared to the circuit simulators such as SPICE.

==> references.tex <==
@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}

%%%%

@article{hsieh2019learning,
  title={Learning neural PDE solvers with convergence guarantees},
  author={Hsieh, Jun-Ting and Zhao, Shengjia and Eismann, Stephan and Mirabella, Lucia and Ermon, Stefano},
  journal={arXiv preprint arXiv:1906.01200},
  year={2019}
}

@inproceedings{nguyen2019deep,
  title={A Deep Learning Approach for Volterra Kernel Extraction for Time Domain Simulation of Weakly Nonlinear Circuits},
  author={Nguyen, Thong and Wang, Xinying and Chen, Xu and Schutt-Aine, Jose},
  booktitle={2019 IEEE 69th Electronic Components and Technology Conference (ECTC)},
  pages={1889--1896},
  year={2019},
  organization={IEEE}
}

@inproceedings{zhang2019circuit,
  title={Circuit-GNN: Graph Neural Networks for Distributed Circuit Design},
  author={Zhang, Guo and He, Hao and Katabi, Dina},
  booktitle={International Conference on Machine Learning},
  pages={7364--7373},
  year={2019}
}

@inproceedings{mcconaghy2011high,
  title={High-dimensional statistical modeling and analysis of custom integrated circuits},
  author={McConaghy, Trent},
  booktitle={2011 IEEE Custom Integrated Circuits Conference (CICC)},
  pages={1--8},
  year={2011},
  organization={IEEE}
}

@article{abrishami2020nn,
  title={NN-PARS: A Parallelized Neural Network Based Circuit Simulation Framework},
  author={Abrishami, Mohammad Saeed and Ge, Hao and Calderon, Justin F and Pedram, Massoud and Nazarian, Shahin},
  journal={arXiv preprint arXiv:2002.05292},
  year={2020}
}

@inproceedings{abrishami2019csm,
  title={CSM-NN: Current source model based logic circuit simulation-a neural network approach},
  author={Abrishami, Mohammad Saeed and Pedram, Massoud and Nazarian, Shahin},
  booktitle={2019 IEEE 37th International Conference on Computer Design (ICCD)},
  pages={393--400},
  year={2019},
  organization={IEEE}
}

@article{peng2020dnn+,
  title={DNN+ NeuroSim V2. 0: An End-to-End Benchmarking Framework for Compute-in-Memory Accelerators for On-chip Training},
  author={Peng, Xiaochen and Huang, Shanshi and Jiang, Hongwu and Lu, Anni and Yu, Shimeng},
  journal={arXiv preprint arXiv:2003.06471},
  year={2020}
}

@inproceedings{he2019noise,
  title={Noise injection adaption: End-to-end ReRAM crossbar non-ideal effect adaption for neural network mapping},
  author={He, Zhezhi and Lin, Jie and Ewetz, Rickard and Yuan, Jiann-Shiun and Fan, Deliang},
  booktitle={Proceedings of the 56th Annual Design Automation Conference 2019},
  pages={1--6},
  year={2019}
}

@article{jain2018rxnn,
  title={RxNN: A Framework for Evaluating Deep Neural Networks on Resistive Crossbars},
  author={Jain, Shubham and Sengupta, Abhronil and Roy, Kaushik and Raghunathan, Anand},
  journal={arXiv preprint arXiv:1809.00072},
  year={2018}
}

@inproceedings{sill1998monotonic,
  title={Monotonic networks},
  author={Sill, Joseph},
  booktitle={Advances in neural information processing systems},
  pages={661--667},
  year={1998}
}

@article{dugas2009incorporating,
  title={Incorporating functional knowledge in neural networks},
  author={Dugas, Charles and Bengio, Yoshua and B{\'e}lisle, Fran{\c{c}}ois and Nadeau, Claude and Garcia, Ren{\'e}},
  journal={Journal of Machine Learning Research},
  volume={10},
  number={Jun},
  pages={1239--1262},
  year={2009}
}

@article{zhou2020noisy,
  title={Noisy Machines: Understanding Noisy Neural Networks and Enhancing Robustness to Analog Hardware Errors Using Distillation},
  author={Zhou, Chuteng and Kadambi, Prad and Mattina, Matthew and Whatmough, Paul N},
  journal={arXiv preprint arXiv:2001.04974},
  year={2020}
}

@inproceedings{angizi2019accelerating,
  title={Accelerating Deep Neural Networks in Processing-in-Memory Platforms: Analog or Digital Approach?},
  author={Angizi, Shaahin and He, Zhezhi and Reis, Dayane and Hu, Xiaobo Sharon and Tsai, Wilman and Lin, Shy Jay and Fan, Deliang},
  booktitle={2019 IEEE Computer Society Annual Symposium on VLSI (ISVLSI)},
  pages={197--202},
  year={2019},
  organization={IEEE}
}

@article{dockhorn2019discussion,
  title={A discussion on solving partial differential equations using neural networks},
  author={Dockhorn, Tim},
  journal={arXiv preprint arXiv:1904.07200},
  year={2019}
}

@misc{chaeun2020spyce,
  author = {Chaeun Lee},
  title = {SPYCE},
  year = {2020},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/chaeunl/SPYCE}},
  commit = {}
}

@misc{maltae2020aihwkit,
 author = {Malte J. Rasch and Diego Moreda and Tayfun Gokmen and others},
 title = {IBM Analog Hardware Acceleration Kit},
 year = {2021},
 publisher = {GitHub},
 journal = {GitHub repository},
 howpublished = {\url{https://github.com/IBM/aihwkit}},
 commit = {543af50b0daf9949e601734c5f9a0bbbd74da28f}

}

@article{roy2020txsim,
  title={TxSim: Modeling Training of Deep Neural Networks on Resistive Crossbar Systems},
  author={Roy, Sourjya and Sridharan, Shrihari and Jain, Shubham and Raghunathan, Anand},
  journal={arXiv preprint arXiv:2002.11151},
  year={2020}
}

@inproceedings{chen2018neural,
  title={Neural ordinary differential equations},
  author={Chen, Ricky TQ and Rubanova, Yulia and Bettencourt, Jesse and Duvenaud, David K},
  booktitle={Advances in neural information processing systems},
  pages={6571--6583},
  year={2018}
}

@article{chakraborty2020geniex,
  title={GENIEx: A Generalized Approach to Emulating Non-Ideality in Memristive Xbars using Neural Networks},
  author={Chakraborty, Indranil and Ali, Mustafa Fayez and Kim, Dong Eun and Ankit, Aayush and Roy, Kaushik},
  journal={arXiv preprint arXiv:2003.06902},
  year={2020}
}

@article{chakraborty2020resistive,
  title={Resistive crossbars as approximate hardware building blocks for machine learning: Opportunities and challenges},
  author={Chakraborty, Indranil and Ali, Mustafa and Ankit, Aayush and Jain, Shubham and Roy, Sourjya and Sridharan, Shrihari and Agrawal, Amogh and Raghunathan, Anand and Roy, Kaushik},
  journal={Proceedings of the IEEE},
  volume={108},
  number={12},
  pages={2276--2310},
  year={2020},
  publisher={IEEE}
}

@inproceedings{gupta2017steam,
  title={STEAM: Spline-based tables for efficient and accurate device modelling},
  author={Gupta, Archit and Wang, Tianshi and Gokcen, Ahmet Mahmutoglu and Roychowdhury, Jaijeet},
  booktitle={2017 22nd Asia and South Pacific Design Automation Conference (ASP-DAC)},
  pages={463--468},
  year={2017},
  organization={IEEE}
}

@inproceedings{kim2019vcam,
  title={VCAM: Variation Compensation through Activation Matching for Analog Binarized Neural Networks},
  author={Kim, Jaehyun and Lee, Chaeun and Kim, Jihun and Kim, Yumin and Hwang, Cheol Seong and Choi, Kiyoung},
  booktitle={2019 IEEE/ACM International Symposium on Low Power Electronics and Design (ISLPED)},
  pages={1--6},
  year={2019},
  organization={IEEE}
}

@inproceedings{liao2018defense,
  title={Defense against adversarial attacks using high-level representation guided denoiser},
  author={Liao, Fangzhou and Liang, Ming and Dong, Yinpeng and Pang, Tianyu and Hu, Xiaolin and Zhu, Jun},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1778--1787},
  year={2018}
}

@inproceedings{nguyen2018transient,
  title={Transient simulation for high-speed channels with recurrent neural network},
  author={Nguyen, Thong and Lu, Tianjian and Sun, Ju and Le, Quang and We, Ken and Schut-Aine, Jose},
  booktitle={2018 IEEE 27th Conference on Electrical Performance of Electronic Packaging and Systems (EPEPS)},
  pages={303--305},
  year={2018},
  organization={IEEE}
}

@article{wang2019massive,
  title={Massive computational acceleration by using neural networks to emulate mechanism-based biological models},
  author={Wang, Shangying and Fan, Kai and Luo, Nan and Cao, Yangxiaolu and Wu, Feilun and Zhang, Carolyn and Heller, Katherine A and You, Lingchong},
  journal={Nature communications},
  volume={10},
  number={1},
  pages={1--9},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{meena2014overview,
  title={Overview of emerging nonvolatile memory technologies},
  author={Meena, Jagan Singh and Sze, Simon Min and Chand, Umesh and Tseng, Tseung-Yuen},
  journal={Nanoscale research letters},
  volume={9},
  number={1},
  pages={526},
  year={2014},
  publisher={Springer}
}
